Self-Adaptive Reconfigurable Arrays (SARA): Using ML to Assist Scaling GEMM Acceleration

With increasing diversity in Deep Neural Network(DNN) models in terms of layer shapes and sizes, the research community has been investigating flexible/reconfigurable accelerator substrates. This line of research has opened up two challenges. The first is to determine the appropriate amount of flexibility within an accelerator array that that can trade-off the performance benefits versus the area overheads of the reconfigurability. The second is being able to determine the right configuration of the array for the current DNN model and/or layer and reconfigure the accelerator at runtime. This work introduces a new class of accelerators that we call Self Adaptive Reconfigurable Array (SARA). SARA architectures comprise of both a reconfigurable array and a hardware unit capable of determining an optimized configuration for the array at runtime. We demonstrate an instance of SARA with an accelerator we call SAGAR, which introduces a novel reconfigurable systolic array that can be configured to work as a distributed collection of smaller arrays of various sizes or as a single array with flexible aspect ratios. We also develop a novel recommendation neural network called ADAPTNET which recommends an array configuration and dataflow for the current layer parameters. ADAPTNET runs on an integrated custom hardware ADAPTNETX that runs ADAPTNET at runtime and reconfigures the array, making the entire accelerator self-sufficient. SAGAR is capable of providing the same mapping flexibility as a collection of 1024 4x4 arrays working as a distributed system while achieving 3.5x more power efficiency and 3.2x higher compute density Furthermore, the runtime achieved on the recommended parameters from ADAPTNET is 99.93% of the best achievable runtime.

==> introduction-micro.tex <==
\section{Introduction}

General Matrix to Matrix Multiplication (GEMM) is at the heart of Deep Learning (DL) training and inference and thus has been the target application of many recent accelerator designs~\cite{eyeriss, tpu, brainwave, zhang-fpga-2015, tetris, tangram}.
As DL becomes pervasive and models become larger, scaling the size of accelerators is a natural next research step.

In general, there are two ways to scale GEMM accelerators. The first, often called ``scale-up", involves adding more compute and memory to a monolithic array. The second, often called ``scale-out", involves creating a distributed set of small arrays connected by a network-on-chip/network-on-package. Unfortunately, neither approach is optimal across all workloads~\cite{scalesim-ispass}. 
\autoref{fig:scale-out-example-intro-new} illustrates this with two toy GEMM workloads.

% (depicted as Rigid Monolithic in \autoref{fig:scale-out-example-intro-new}). The second, often called ``scale-out", involves creating a distributed set of small arrays connected by a network-on-chip/network-on-package (shown as Distributed in \autoref{fig:scale-out-example-intro-new}).
% Unfortunately, neither approach is optimal across all workloads~\cite{scalesim-ispass}. 


Scaling-up rigid arrays (depicted as \textit{Rigid Monolithic} in \autoref{fig:scale-out-example-intro-new}) 
can often lead to under-utilization when the dimensions of the 
GEMM do not align with the aspect ratio of the array (\textit{irregular workload} in \autoref{fig:scale-out-example-intro-new}).
Current solutions to address this issue have advocated for expensive non-blocking 
networks-on-chip (e.g.,
fat-trees, butterflies and benes) 
betweeen the 
SRAMs and PEs~\cite{maeri, sigma} to provide flexibility (depicted as \textit{Flexible Monolithic} in \autoref{fig:scale-out-example-intro-new}). 
Unfortunately, while this can help enhance mapping utilization, it comes at a significant area and power cost\footnote{non-blocking topologies are known to scale as O(NlogN) to O(N$^2$) with the number of end-points} and limits scalability. 

Yet another problem with reconfigurable 
flexible architectures 
is the cost to find optimal architecture configurations for the given workload.
All prior works on reconfigurable accelerators rely on a compiler/mapper to determine the optimal configuration via exhaustive, heuristic or optimization algorithm-based searches~\cite{timeloop, gamma, zhao2019mrna}.
Deploying such a design therefore has a couple of challenges: (i) a cost model has be to developed and integrated into the software stack to help find optimal mappings, without which the flexible design loses utility,
(ii) an expensive configuration and mapping search has to be performed at compile-time before scheduling any workload. Usually mapping search in software takes about a few seconds to hours~\cite{timeloop, gamma, zhao2019mrna}, even with sophisticated ML assisted frameworks like autoTVM \cite{autotvm}.

As an alternative, scaling out (shown as \textit{Distributed} in \autoref{fig:scale-out-example-intro-new}) 
can help mitigate the under-utilization challenge, since irregular GEMMs can be tiled on to the smaller arrays as \autoref{fig:scale-out-example-intro-new} shows. 
However, this leads to loss in 
spatial reuse (i.e., direct data-forwarding) that scale-up designs provide, 
and also requires data replication across the SRAMs of the individual arrays.
Data replication leads to a decrease in overall on-chip storage capacity, leading to a loss of temporal reuse due to smaller tiles.
Moreover, distributed arrays can exacerbate the mapping search problem~\cite{simba, timeloop}.
%\TODO{add that distributed needs mapping search}

We propose a solution to address 
all the challenges listed above. Specifically,
we make three contributions.

%describe three contributions to address these problems.


\insertFigure{scale-out-example-intro-new}{Comparison of scalability, utilization, and operand reuse in traditional monolithic and distributed accelerators, and the position of the proposed architecture}

\insertFigure{sara-concept}{
    The constitution and interactions of the self adaptive (SA) and reconfigurable array (RA) components to make up the SARA accelerator called \mys{} in this work. 
}


\textit{First contribution:} A novel accelerator architecture called \textsc{Reconfigurable Systolic Array} (\ra) that can be configured to operate in both scale-up and scale-out settings by adding light-weight configurability within a traditional systolic array. 
The \ra~is capable of realizing all mappings as in distributed configuration, without losing spatial reuse. 
Moreover, unlike a distributed configuration with fixed array dimensions and fixed parts, the \ra~can be configured to have variable array dimensions and number of sub-arrays as depicted later in \autoref{fig:high-bw-smart-systolic-array}(d).
In practice, \ra~closely approximates a flexible monolithic design, with a fraction of area cost.
\autoref{fig:scale-out-example-intro-new} shows our \ra provides utilization, reuse, and scalability.

\textit{Second contribution:} We develop a novel ML model called \recnet{} which we train to learn and generalize the configuration space of \ra{}. 
In contrast to existing methods, \recnet{} enables a O(1) recommendation of the accelerator configuration given any workload, avoiding any search.
%\TK{we need to explain the following line better. reviewers might wonder what we mean by best runtime and whether 99.93 is accuracy}. 
The recommendations from \recnet{} on average (GeoMean), achieve  99.93\% of the best possible runtime (oracle) in our tests with 200K samples (\autoref{fig:sara-system}(c)). 

\textit{Third contribution}: We present a custom hardware engine for running \recnet, called \core. The custom design of \core~ enables it to
generate both the optimal mapping and architecture configuration for any workload being run on \ra{} 
in approximately 600 cycles, which is at least about 6 orders of magnitude faster than software.
Furthermore, \core{} consumes the same hardware real-estate and roughly the same on-chip memory capacity
\footnote{The only change in \recnet{} between various \ra{} is the weight of the output layer, which is small in comparison to the embedding table which takes most of the on-chip space}
for different arrays and with number of workloads,
%\TK{doesn't on-chip memory capacity of \core{} depend on size of \ra{}?} 
thus proving to be a scalable solution in contrast to approaches like using configuration caches.
With \core{} the configuration lookup using \recnet{} can be performed at runtime, without involving the software stack.

Together, these three components enable us to develop 
a new class of accelerators that we call \textit{Self Adaptive Reconfigurable Array (SARA)} (\autoref{fig:sara-concept}). 
SARA accelerators can self adapt at runtime to optimized configurations for the target workload, without 
requiring compile-time analysis.
%We integrate these three components into an accelerator
We demonstrate an instance of SARA that we name `Shape Adaptive GEMM AcceleratoR (\mys{} \footnote{Sagar is a Sanskrit word that means Ocean, reflecting the ability of our accelerator to have flexible shapes})' as shown in \autoref{fig:sara-concept}
and evaluate its performance across various %baseline 
configurations.
 %
We show that \mys{} has 
3.2$\times$ higher compute density and
3.5$\times$ improved power efficiency, over equivalent scaled-out systolic array.
%
The extra flexibility costs $<$10\% in area and 
50\% in power, compared to equivalent scaled-up systolic array.
%
Compared to an area normalized state-of-the-art flexible scalable accelerator \cite{sigma}, \mys~ incorporates 
45\% more compute.
When comparing compute-equivalent configurations,
\mys~ consumes 43\% less power and 30\% less area.

%We believe our proposed accelerator is the first in a class of designs we name \textit{Self Adaptive Reconfigurable Array (SARA)} (\autoref{fig:sara-concept}).
To summarize, we make the following contributions.
(i) We propose \textbf{\ra}, a reconfigurable architecture for scalable GEMM acceleration, simultaneously achieving high utilization and reuse.
(ii) We develop \textbf{\recnet}, a lean recommendation neural net which suggests optimized configuration and dataflow 
%at constant time 
with high accuracy.
(iii) We implement \textbf{\core}, a hardware capable of running \recnet{} in constant time and configuring \ra{} at runtime.
(iv) We integrate the above components into a SARA accelerator called \textbf{\mys{}}, which achieves optimal runtime at lower power and area than SOTA.



\begin{comment}
General Matrix to Matrix Multiplication (GEMMs) is at the heart of Deep Learning (DL) training and inference and thus has been the target application of many accelerator designs~\cite{eyeriss, tpu, brainwave, zhang-fpga-2015, tetris, tangram}.
However these individual devices work on small matrix tiles, and do not have enough computation power to work on larger networks without multiple costly passes. 
Recent proposals \cite{tangram}\cite{simba} have demonstrated the need for scaling the DNN computation engines to meet the computation demands of contemporary workloads. 
Despite extensive research and product development on architectures for small-tile GEMMs, designing efficient architectures for performing \textit{GEMMs at scale} is still non-trivial.

The crux of the problem is that there exists a pernicious trade-off between \textit{scalability} and \textit{utilization} (or mapping efficiency).
Scalability is a direct consequence of simplicity and regularity of a particular design.
For instance, regular designs like the TPU~\cite{tpu} (systolic array) can pack large number of MAC units (e.g., $128\times128$ in TPUv3) 
in a reasonable power and area budget. 
Utilization, on the other hand, requires 
mapping flexibility since GEMMs are often irregular in practice~\cite{sigma} and may 
not match the dimensions of the physical array.
%This is because irregular GEMM dimensions are more of a norm than exception \cite{sigma}.
%, this cost seems to be a necessary evil. 
There are two ways of achieving such flexibility.
The first is to provide rich connectivity
for operand distribution and output collection within the array. This has been demonstrated in proposals like MAERI~\cite{maeri} and SIGMA~\cite{sigma} that use all-to-all interconnects to enhance utilization.
This, however, comes at the cost of high area-power costs, 
which is at direct odds with scalability.
The alternate approach is to design 
an accelerator as a 
distributed \emph{scaled out}\footnote{
We use scale-up/scale-out interchangeably with monolithic/distributed.
} collection of smaller sub-accelerators, which is further corroborated by recent architecture proposals \cite{simba, tangram}. However, this leads to loss of operand reuse opportunities between the sub-accelerators.
\end{comment}
%
% Given that irregular workload dimensions are more of a norm than exception \cite{sigma}, this cost seems to be a necessary evil. 
% %
% However, a recent study ~\cite{scalesim-ispass} argues that a distributed \emph{scaled out}\footnote{
% We use scale-up/scale-out interchangeably with monolithic/distributed.
% }
% setting is a feasible alternative to gain flexibility, which is further corroborated by recent architecture proposals \cite{simba, tangram}.

\begin{comment}
\insertFigure{scale-out-example-intro}{Challenges in efficiently scaling GEMM arrays.
             (i) In case of irregular matrix dimensions, a monolithic configuration under performs due to mapping inefficiency, while a distributed configuration achieves max performance.
             (ii) For regular matrix dimensions, both the arrays achieve similar performance, but the distributed configuration suffers from poor operand reuse. \TK{I think it'll be better to show monolithic on left and distributed on right instead of organizing based on workload. Also the text inside the brown and blue/green boxes is not visible at all -- make the color lighter and increase font size. Scale-up (Rigid) : 
Scale-up (Flexible): 
Scale-out 
Scale-* (This work). And add boxes for Wire Scalability, Utilization and Operand Reuse. Come up with three examples, one that is bad for distributed.
}
}
\end{comment}


\begin{comment}
\insertFigure{scale-out-example-intro-new}{Caption TBD}

\TK{lets discuss three choices here: Scale-up (Rigid) : 
Scale-up (Flexible), and scale-out. And lead this up to our proposal which is Scale-*?}
\autoref{fig:scale-out-example-intro} sheds light into the trade-off space.
In the case of irregular matrix dimensions (case (i)), the monolithic array is unable to extract full performance, due to mapping inefficiencies, while the distributed configuration has no such limitation. 
However, the distributed configuration is unable to extract the benefits of operand reuse. 
This makes the choice of distributed configurations inferior to a monolithic array, where matrices with regular dimensions are involved, as shown in case (ii).
%
The loss of spatio-temporal operand reuse is a consequence of two factors. 
First, spatial reuse via wires is lost since communication paths between two distinct compute units are fundamentally lower-bandwidth than  within the array---in the worst case requiring off-chip access~\cite{simba}.
Second, some operand data is needed to be replicated in the local storage of each device (case (ii)), which reduces the effective on-chip capacity. 
This reduced capacity leads to loss of temporal reuse and results in increased off-chip accesses.
These factors make a distributed configuration inferior in energy efficiency.

\insertFigure{sara-concept}{
    The constitution and interactions of the self adaptive (SA) and reconfigurable array (RA) components to make up the SARA accelerator called \mys{} in this work. \TK{change SMART systolic Array to Reconfigurable Systolic Array}
}

\textbf{Contribution 1:} In this paper, we propose a novel accelerator micro-architecture organization called \textsc{SmartSystolic} Array (\ra{}) aimed to attain the benefits of monolithic (i.e., scale-up) and distributed (i.e., scale-out) designs for efficient GEMM computation in a single unified substrate. 
We choose systolic arrays as our scale-up building blocks, since the simplicity of these arrays leads to low area and power overheads, maximizing local bandwidth while minimizing communication distance.
To mitigate the under-utilization problem, we propose augmenting the traditional systolic design with a bypass interconnection network inspired by SMART \cite{smart}. 
%
These links permits us to emulate similar mapping to a distributed cluster of accelerator, within a monolithic compute array. The bypass interconnect can also be configured to emulate distributed systems of different granularities, eg. a system with $128\times128$ MAC (multiply and accumulate units) can be configured to be used as 4 $64\times64$ units or 16 $32\times32$ units or even 32 $32\times16$ units.


\textbf{Contribution 2: }
Determining the optimal architecture configuration and mapping strategy for each workload (eg. each layer in a DNN) is critical to obtain the performance and energy benefits from a reconfigurable array. 
Currently such architectures solely rely on software for this task. 
The software methods~\cite{timeloop, gamma, autotvm} are constrained to operate in a static setting, since their runtimes are in the order of a few seconds to hours. 
Furthermore, the complete reliance on software also hinders the deployability of such new architectures, as a significant effort is needed to update the software stack to incorporate the cost model and configuration search capability.
%
In this work, we aim to reduce this cross-stack dependency by incorporating a reconfiguration unit called \textit{Self Adaptive (SA)} unit (see \autoref{fig:sara-concept}), which is capable of predicting the optimal configuration as the workloads arrive at runtime.
%
We developed a novel light weight neural recommendation model called \recnet, to recommend the optimal configuration of the array depending on the incoming workload at runtime.
The recommender is capable of predicting attain about 99.93\% of the best runtime on average (GeoMean) in our tests with 200K samples.


\textbf{Contribution 3: }
We also design a custom hardware for running \recnet, called \core, and augment it with the reconfigurable accelerator.
The custom design of \core~ enables the SA unit to generate both the optimal mapping and hardware configuration in approximately 600 cycles, which is at least about 6 orders of magnitude faster than software.   
The resulting design is self sufficient for providing optimal performance. 
Furthermore, the SA unit consume the same hardware real-estate and on-chip memory capacity for different arrays and with number of workloads thus proving to be a scalable solution in contrast to approaches like using configuration caches.

\textbf{Contribution 4: }
We integrate these three components into an accelerator which we call `Shape Adaptive GEMM AcceleratoR (\mys{} \footnote{Sagar is a Sanskrit word that means Ocean, reflecting the ability of our accelerator to have flexible shapes})' as shown in \autoref{fig:sara-concept}
and evaluate its performance across various %baseline 
configurations.
 %
We show that \mys{} has 
3.2$\times$ higher compute density and
3.5$\times$ improved power efficiency, over equivalent scaled-out systolic array.
%
The extra flexibility costs $<$10\% in area and 
50\% in power, compared to equivalent scaled-up systolic array.
%
Compared to an area normalized state-of-the-art flexible scalable accelerator \cite{sigma}, \mys~ incorporates 
45\% more compute, 
while when comparing compute-equivalent configurations,
\mys~ consumes 43\% less power 
and saves 30\% area.


We believe our proposed accelerator is the first in a class of designs we name \textit{Self Adaptive Reconfigurable Array (SARA)} (\autoref{fig:sara-concept}).
To summarize, we make the following contributions.
%\todo{Here flip the order, ie. introduce sara via model-M, and then mention the two sub components}
%In this paper we make the following contributions.
(i) We propose \textbf{\ra}, a reconfigurable architecture for scalable GEMM acceleration, simultaneously achieving high utilization and reuse.
(ii) We develop \textbf{\recnet}, a lean recommendation neural net which suggests optimized configuration and dataflow 
%at constant time 
with high accuracy.
(iii) We implement \textbf{\core}, a hardware capable of running \recnet{} in constant time and configuring \ra{} at runtime.
(iv) We integrate the above components into a SARA accelerator called \textbf{\mys{}}, which achieves optimal runtime at lower power and area than SOTA.
\end{comment}

%(iii) Demonstrate \textbf{Self Adaptive  Reconfigurable Architecture (SARA)} as a reference design \mys, which achieves optimal runtime at lower power and area than state of the art.

\begin{comment}
\item{We develop a neural network recommendation engine, which can predict the most performant architecture and mapping configuration per workload, at runtime with very high accuracy. 
To the best of our knowledge this is the first work to do so.}
\item{We demonstrate the first instance of a Self Adaptive  Reconfigurable Architecture (SARA); a class of architectures capable of independently selecting and implementing the most optimal configuration for a given workload at runtime.}
\squishend
\end{comment}

==> related-works.tex <==
\vspace{-2mm}
\section{Related Works}
\label{sec:related-work}
%\vspace{-2mm}

% Moved to section 2
%\input{tables/related-works-table}

%\textcolor{red}{Need to add planaria, other recommendation system based work- DAC work by Luca Carloni}

%\TK{This section can be shortened. I recommend (:p) keeping it crisp and dividing it into three categories: (i) reconfigurable DNN accelerators, (ii) dataflow and arch design-space exploration - cite some of the tools like SCALE-sim, Timeloop, dMazeRunner, Marvel that let you do exhaustive/heuristic-based searches for accelerator configuration and/or mappings. And mention that they cannot find optimal configs at runtime like RecNet does, (iii) ML-assisted system configuration - cite works like Google's RL based task placement, AutoTVM that uses ML inside compiler, and so on. GAMMA paper's related work has some of these listed}

\textbf{Flexible DNN Accelerator}.
% Anand: Uncomment in camera ready
\autoref{table:related-works} depicts the standing of various such accelerators in term of native operation supported, mapping capability and flexibility.
To efficiently execute a variety of workloads, DNN accelerator designs generally come with two tiers of flexibility, architecture and dataflow.
Designs like Neurocube\cite{neurocube}, Flexflow\cite{flexflow}, and by FPGA based designs\cite{zhang-fpga-2015} enable flexible mapping by supporting multiple dataflow. 
On the other hand proposals like Planaria \cite{planaria}, Brainwave\cite{brainwave}, SIGMA \cite{sigma}, MAERI\cite{maeri}, Cascades\cite{cascades} and others \cite{zhang-fpga-2015, alwani-2016-MICRO-fused, tangram} enable reconfiguration at the hardware level.
\ra{} enables both mapping flexibility and reconfigurability.

\textbf{Dataflow and Accelerator Design Space Search.} Several architecture and mapping space exploration tools have been proposed in the recent past to take advantage of flexibilities in the design. 
Tool like SCALE-Sim\cite{scalesim-ispass}, MAESTRO\cite{maestro}, Tetris\cite{tetris} etc. provide analytical models for fast cost estimation of specific configurations. 
While Timeloop\cite{timeloop}, dMazeRunner\cite{dmazerunner} etc are tools which perform heuristic or exhaustive search for architecture configuration or mapping strategy. 
SARA systems like \mys{} on the other hand use a trained recommender like \recnet{} to circumvent the search and obtain the optimal configuration and dataflow in one shot at runtime.

\textbf{ML assisted system configuration.} Recent works have demonstrated the use of ML algorithms to assist in system configuration. 
%
Gamma\cite{gamma} and ConfuciuX\cite{confuciux} perform architecture mapping and design space configuration search using genetic algorithm and reinforcement learning (RL).
On more systems size, work by 
Mirhoseni et al\cite{mirhoseini2017device} use RL for task placement on a heterogenous system, while modern compilers like AutoTVM\cite{autotvm} use ML models for cost prediction to improve compilation time.
Nautilus\cite{nautilus} uses genetic algorithm to improve FPGA place and route.
It is worth noting that these approaches mostly enhance search for the optimal configuration, and this unlike \recnet{} do not replace search.
Perhaps the closest to our approach is work by Kwon et al\cite{kwon2019learning}, who use online tensor-based recommender systems to aid place and route in chip design.

==> tables/scaling-table.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\newcommand{\multarr}[0]{\begin{tabular}{c} Multiple \\ Arrays \end{tabular}}
\newcommand{\vararr}[0]{\begin{tabular}{c} Variable \\ arrays sizes \end{tabular}}
\newcommand{\flexdim}[0]{\begin{tabular}{c} Flexible \\ array dimensions \end{tabular}}

\newcommand{\accnames}[0]{\begin{tabular}{c} TPU \\ MAERI \\ Simba \\ Tangram \\ SIGMA \end{tabular}}
\newcommand{\scalabiltymarks}[0]{\begin{tabular}{P{2.5cm}P{3.3cm}}
                                        \checkmark & \xmark \\ 
                                        \xmark & \checkmark \\ 
                                        \checkmark & \xmark \\ 
                                        \xmark & \checkmark \\ 
                                        \xmark & \checkmark 
                                \end{tabular}}
                                                                
\newcommand{\utilmarks}[0]{\begin{tabular}{P{1.5cm}P{3cm}P{3CM}}
                                        \xmark & \xmark & \xmark \\ 
                                        \xmark & \checkmark & \checkmark \\ 
                                        \checkmark & \xmark & \xmark \\
                                        \checkmark & \xmark & \xmark \\ 
                                        \checkmark & \xmark & \xmark 
                                \end{tabular}}

\begin{table}[t] 
\centering 
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{0pt} 
\caption{\textit{ Caption TBD. \TK{add SAGAR as row at the bottom with all checks}}} 
\Large
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|c|c}
            & Ease of Scalability & Ease of Maximizing Utilization \\
        \hline
            & \begin{tabular}{P{2.5cm}|P{3.3cm}} Wire Area & Operand Reuse \end{tabular}
            & \begin{tabular}{c|c|c} \multarr & \vararr & \flexdim \end{tabular} \\
        \hline
        
        \accnames & \scalabiltymarks & \utilmarks \\
        
        \hline
        
    \end{tabular}
}
\label{table:scaling-motivation} 
\end{table}

